Human Motion Modeling using DVGANs

We present a novel generative model for human motion modeling using Generative Adversarial Networks (GANs). We formulate the GAN discriminator using dense validation at each time-scale and perturb the discriminator input to make it translation invariant. Our model is capable of motion generation and completion. We show through our evaluations the resiliency to noise, generalization over actions, and generation of long diverse sequences. We evaluate our approach on Human 3.6M and CMU motion capture datasets using inception scores.

==> figure/ablation.tex <==
\begin{table*}[!htbp]
\centering
\begin{tabular}{ l |c c c c | c |c c c c }
\toprule
\multicolumn{10}{c}{\textbf{CMU Mocap $N=32$ $f=4\text{Hz}$}}\\
\midrule
Generator	&Validation	& Noise	& Data	& Final & Inception & \multicolumn{4}{c}{Action Retrieval} \\
			&  			&		& Aug. 	& Cut 	& Score & R@1 	& R@3 	& R@5 	& R@10 	\\
\midrule
CNN		& final	& all	&			&		&	y	&	-	&	-	&	-	&	-	\\
CNN		& mod 2	& all	&			&		&	y	&	-	&	-	&	-	&	-	\\
CNN		& all	& first	&			&		&	n	&	-	&	-	&	-	&	-	\\
CNN		& all	& mod 2	&			&		&	n	&	-	&	-	&	-	&	-	\\
CNN		& all	& all	&			&		&	y	&	-	&	-	&	-	&	-	\\
CNN		& all	& all	&	x		&		&	y	&	-	&	-	&	-	&	-	\\
CNN		& all	& all	&	x		&	x	&	y	&	-	&	-	&	-	&	-	\\
\midrule
RNN		& final	& all	&			&		&	n	&	-	&	-	&	-	&	-	\\
RNN		& mod 2	& all	&			&		&	n	&	-	&	-	&	-	&	-	\\
RNN		& all	& first	&			&		&	n	&	-	&	-	&	-	&	-	\\
RNN		& all	& mod 2	&			&		&	n	&	-	&	-	&	-	&	-	\\
RNN		& all	& all	&			&		&	n	&	-	&	-	&	-	&	-	\\
RNN		& all	& all	&	x		&		&	y	&	-	&	-	&	-	&	-	\\
RNN		& all	& all	&	x		&	x	&	n	&	-	&	-	&	-	&	-	\\
\midrule
\multicolumn{2}{c}{Real video samples} & &	 &	&	-	&	-	&	-	&	-	&	-	\\
\midrule
\bottomrule
\end{tabular}
\caption{Ablation study}
\label{table:ablation}
\end{table*}


==> figure/motion_prediction_4col.tex <==
\begin{table*}[!htbp]
\centering
\begin{tabular}{ l |c c c c |c c c c | c c c c | c c c c}
\toprule
\multicolumn{17}{c}{H3.6M motion prediction with 50 initial frames}\\
\midrule
			& \multicolumn{4}{c}{Walking} 	&  \multicolumn{4}{c}{Eating} 	& \multicolumn{4}{c}{Smoking} 	&  \multicolumn{4}{c}{Discussion} 		\\
Approach	& 80	& 160	& 320	& 400 	&  80	& 160	& 320	& 400  & 80	& 160	& 320	& 400	&  80	& 160	& 320	& 400 \\
\midrule
ERD~\cite{FragkiadakiLM15}				& 0.93	& 1.18	& 1.59	& 1.78	& 1.27	&  1.45	& 1.66	& 1.80 	& 1.66	& 1.95	& 2.35	& 2.42	& 2.27	&  2.47	& 2.68	& 2.76	\\
LSTM-3LR~\cite{FragkiadakiLM15}			& 0.77	& 1.00	& 1.29	& 1.47	& 0.89	& 1.09	& 1.35	& 1.46 	& 1.34	& 1.65	& 2.04	& 2.16	& 1.88	& 2.12	& 2.25	& 2.23 	\\
SRNN~\cite{JainZSS16}					& 0.81	& 0.94	& 1.16	& 1.30	& 0.97	& 1.14	& 1.35	& 1.46 	& 1.45	& 1.68	& 1.94	& 2.08	& 1.22	& 1.49	& 1.83	& 1.93 \\
Residual sup. MA~\cite{MartinezBR17}	& 0.28	& 0.49	& 0.72	& 0.81	& 0.23	& 0.39	& 0.62	& 0.76 	& 0.33	& 0.61	& 1.05 	& 1.15	& 0.31	& 0.68	& 1.01	& 1.09 	\\
Zero-velocity							& 0.39	& 0.68	& 0.99	& 1.15	& 0.27	& 0.48	& 0.73	& 0.86 	& 0.26	& 0.48	& 0.97	& 0.95	& 0.31	& 0.67	& 0.94	& 1.04 	\\
\midrule
Our RNN-GAN								& 0.36	& 0.59 	& 0.89	& 1.00	& 0.39	& 0.61 	& 1.01 	& 1.20 	& 0.28	& 0.49	& 0.85	& 0.97	& 0.50	& 0.86	& 1.31	& 1.53	\\
\bottomrule
\end{tabular}
\caption{\todo{Say something about this table when results are filled in.}}
\label{table:prediction}
\end{table*}
